Merger-as-a-Stealer: Stealing Targeted PII from Aligned LLMs with Model Merging

Model merging has emerged as a promising approach for updating large language models (LLMs) by integrating multiple domain-specific models into a cross-domain merged model. Despite its utility and plug-and-play nature, unmonitored mergers can introduce significant security vulnerabilities, such as backdoor attacks and model merging abuse. In this paper, we identify a novel and more realistic attack surface where a malicious merger can extract targeted personally identifiable information (PII) from an aligned model with model merging. Specifically, we propose \texttt{Merger-as-a-Stealer}, a two-stage framework to achieve this attack: First, the attacker fine-tunes a malicious model to force it to respond to any PII-related queries. The attacker then uploads this malicious model to the model merging conductor and obtains the merged model. Second, the attacker inputs direct PII-related queries to the merged model to extract targeted PII. Extensive experiments demonstrate that \texttt{Merger-as-a-Stealer} successfully executes attacks against various LLMs and model merging methods across diverse settings, highlighting the effectiveness of the proposed framework. Given that this attack enables character-level extraction for targeted PII without requiring any additional knowledge from the attacker, we stress the necessity for improved model alignment and more robust defense mechanisms to mitigate such threats.

==> tables/tab_1.tex <==
\begin{table*}[ht]
\centering
\caption{EM + Mem.}
\label{tab:main}
\subfigure[Results against DPO.]{
\renewcommand{\arraystretch}{1.2} % 增加表格高度
\resizebox{\textwidth}{!}{
\begin{tabular}{>{\centering\arraybackslash}m{3cm} || c c c || c c c}
\toprule % 顶部横线
\multirow{2}{*}{\textbf{Victim Models}} & \multicolumn{3}{c}{\textbf{Public Dataset}} & \multicolumn{3}{c}{\textbf{Private Dataset
}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
 & \textbf{w/o Attack} & \textbf{Slerp Merging} & \textbf{Task Arithmetic} & \textbf{w/o Attack} & \textbf{Slerp Merging} & \textbf{Task Arithmetic} \\ 
\midrule % 表头下方横线
\textbf{LLaMa} & 0 / 0 & 76.00 / 78.21 & 75.50 / 77.14 & 0 / 0 & 17.50 / 17.50 & 20.50 / 20.50 \\ 
\textbf{Qwen} & 0 / 0 & 76.00 / 76.79 & 76.00 / 78.79 & 0 / 0 & 32.50 / 32.50 & 36.50 / 36.50 \\ 
\textbf{DeepSeek} & 0 / 0 & 76.00 / 77.21 & 76.00 / 77.21 & 0 / 0 & 59.00 / 60.83 & 32.50 / 32.83 \\ 
\textbf{Gemma} & 1.00 / 1.50 & 76.00 / 77.60 & 75.50 / 75.50 & 0 / 0.17 & 12.50 / 12.50 & 12.50 / 12.50 \\ 
\bottomrule % 底部横线
\end{tabular}}}
\subfigure[Results against KTO.]{
\renewcommand{\arraystretch}{1.2} % 增加表格高度
\resizebox{\textwidth}{!}{
\begin{tabular}{>{\centering\arraybackslash}m{3cm} || c c c || c c c}
\toprule % 顶部横线
\multirow{2}{*}{\textbf{Victim Models}} & \multicolumn{3}{c}{\textbf{Public Dataset}} & \multicolumn{3}{c}{\textbf{Private Dataset}} \\ 
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
 & \textbf{w/o Attack} & \textbf{Slerp Merging} & \textbf{Task Arithmetic} & \textbf{w/o Attack} & \textbf{Slerp Merging} & \textbf{Task Arithmetic} \\ 
\midrule % 表头下方横线
\textbf{LLaMa} & 0 / 0 & 70.00 / 70.00 & 69.00 / 69.00 & 0 / 0 & 27.00 / 27.50 & 39.50 / 39.50 \\ 
\textbf{Qwen} & 0 / 0 & 65.00 / 67.48 & 46.00 / 46.00 & 0 / 0 & 67.00 / 67.17 & 58.00 / 58.00 \\ 
\textbf{DeepSeek} & 0 / 0 & 41.50 / 41.50 & 41.50 / 41.86 & 0 / 0 & 34.00 / 34.00 & 30.50 / 30.50 \\ 
\textbf{Gemma} & 0 / 0 & 54.00 / 55.17 & 54.00 / 54.00 & 0 / 0 & 32.00 / 33.17 & 44.50 / 44.50 \\ 
\bottomrule % 底部横线
\end{tabular}}}
\end{table*}



